Light meson decays at BESIII

The world's largest sample of $J/\psi$ events accumulated at the BESIII dector offers a unique opportunity to investigate $\eta$ and $\eta^\prime$ physics via two body $J/\psi$ radiative or hadronic decays. In recent years the BESIII experiment has made significant progresses in $\eta/\eta^\prime$ decays. A selection of recent highlights in light meson spectroscopy at BESIII are reviewed in this report, including the observation of $\eta^\prime\rightarrow\pi^+\pi^-\mu^+\mu^-$, the study of $\eta^\prime\rightarrow\pi^+\pi^-e^+e^-$, and search for $CP$-violation in this decay, search for the rare decays of $\eta^\prime\rightarrow4\pi^0$ and $\eta^\prime\rightarrow\gamma\gamma\eta$, as well as the precision measurement of the branching fraction of $\eta^\prime$ decays.

==> abstract.tex <==
The world's largest sample of $J/\psi$ events accumulated at the BESIII dector offers a unique opportunity to investigate $\eta$ and $\eta^\prime$ physics via two body $J/\psi$ radiative or hadronic decays. In recent years the BESIII experiment has made significant progresses in $\eta/\eta^\prime$ decays. A selection of recent highlights in light meson spectroscopy at BESIII are reviewed in this report, including the observation of $\eta^\prime\rightarrow\pi^+\pi^-\mu^+\mu^-$, the study of $\eta^\prime\rightarrow\pi^+\pi^-e^+e^-$, and search for $CP$-violation in this decay, search for the rare decays of $\eta^\prime\rightarrow4\pi^0$ and $\eta^\prime\rightarrow\gamma\gamma\eta$, as well as the precision measurement of the branching fraction of $\eta^\prime$ decays.

